Translating Similar Languages: Role of Mutual Intelligibility in Multilingual Transformers

We investigate different approaches to translate between similar languages under low resource conditions, as part of our contribution to the WMT 2020 Similar Languages Translation Shared Task. We submitted Transformer-based bilingual and multilingual systems for all language pairs, in the two directions. We also leverage back-translation for one of the language pairs, acquiring an improvement of more than 3 BLEU points. We interpret our results in light of the degree of mutual intelligibility (based on Jaccard similarity) between each pair, finding a positive correlation between mutual intelligibility and model performance. Our Spanish-Catalan model has the best performance of all the five language pairs. Except for the case of Hindi-Marathi, our bilingual models achieve better performance than the multilingual models on all pairs.

==> stat_table.tex <==
\begin{table}[h]
\begin{center}
\textbf{Hi-Mr}
\begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|} 
 \hline
\thead{\textbf{Language}} & \thead{\textbf{\#sentences}} & \thead{\textbf{\#words}} \\ 
 \hline
 \hline
hi & 43,274 & 829,976 \\
\hline
mr & 43,274 & 600,006  \\
\hline
mono-hi & 227,167,260 & 4,742,853,278  \\
\hline
mono-mr & 9,975,898 & 331,497,565 \\
\hline 
\hline
\end{tabular}
\textbf{Es-Ca}
\begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|} 
 \hline
\thead{\textbf{Language}} & \thead{\textbf{\#sentences}} & \thead{\textbf{\#words}} \\ 
 \hline
 \hline
ca & 11,379,948 & 162,981,769 \\
\hline
es & 11,379,948 & 150,881,516  \\
\hline
mono-es & 58,416,064 & 1,525,007,410  \\
\hline
mono-ca & 24,745,986 & 763,697,712 \\
\hline 
\hline
\end{tabular}
\textbf{Es-Pt}
\begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|} 
 \hline
\thead{\textbf{Language}} & \thead{\textbf{\#sentences}} & \thead{\textbf{\#words}} \\
es & 4,150,063 & 97,940,590 \\
\hline
pt & 4,150,063 & 94,756,496 \\
\hline
mono-es & 58,416,064 & 1,525,007,410  \\
\hline
mono-pt & 2,016,635 & 50,462,045 \\
\hline
\end{tabular}
\textbf{Sl-Hr}
\begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|} 
 \hline
\thead{\textbf{Language}} & \thead{\textbf{\#sentences}} & \thead{\textbf{\#words}} \\
sl & 17,659,209 & 113,087,914  \\
\hline
hr & 17,659,209 & 117,736,580 \\
\hline
mono-sl & 46,251,729 & 770,646,199 \\
\hline
mono-hr & 64,577,734 & 1,244,102,908 \\
\hline
\end{tabular}
\textbf{Sl-Sr}
\begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|} 
 \hline
\thead{\textbf{Language}} & \thead{\textbf{\#sentences}} & \thead{\textbf{\#words}} \\
sl & 14,130,116 & 79,135,558  \\
\hline
sr & 14,130,116 & 86,152,298 \\
\hline
mono-sl & 46,251,729 & 770,646,199 \\
\hline
mono-sr & 24,073,253 & 489,934,858 \\
\hline
\end{tabular}
\end{center}
\caption{\mam{It's odd to say ``A table showing\dots. You could say: ``Number of sentences\dots"} A table showing the number of sentences and words for the data used for each language pair.}\label{tab:data}
\end{table}
